Task Bias in Vision-Language Models

Incidental supervision from language has become a popular approach for learning generic visual representations that can be prompted to perform many recognition tasks in computer vision. We conduct an in-depth exploration of the CLIP model and show that its visual representation is often strongly biased towards solving some tasks more than others. Moreover, which task the representation will be biased towards is unpredictable, with little consistency across images. To resolve this task bias, we show how to learn a visual prompt that guides the representation towards features relevant to their task of interest. Our results show that these visual prompts can be independent of the input image and still effectively provide a conditioning mechanism to steer visual representations towards the desired task.

==> 01_intro_old.tex <==
\section{Introduction}

Learning visual representations from the synchronization of images and text on the Internet has become a popular technique for performing a variety of visual recognition tasks. Since vision-language models (VLMs) are able to learn the association between a text phrase and an image, a zero-shot classification paradigm has emerged where image classification can be performed by defining the categories with free-form text. Natural language supervision has enabled the field to graduate beyond pre-defined categories and has achieved excellent performance on many recognition benchmarks.

However, language also introduces ambiguity. Fig.~\ref{fig:taskambimg} shows a typical setup for VLMs, where we have an image and a multiple choice set of textual category labels. If you look carefully at the image, you will see there is no clear answer given the information provided. The action being performed is \textit{lift}, the text reads \textit{football}, and the most prominent object is a \textit{weight}. As the label set increases in size, the current VLMs face decisions like this regularly in applied settings. Since the task has not been specified, multiple answers are possible, yet the model can only pick one.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/taskamb_quiz_update.pdf}
    \caption{The CLIP visual representation of this image is strongly predisposed towards solving action recognition over scene text and object recognition.}
    \label{fig:taskambimg}
\end{figure}


We have found that, although the question is unknown, the visual representations have already decided which question to answer solely based on the image.  As shown on the right of Fig.~\ref{fig:taskambimg}, when CLIP is given these choices, it has a strong bias to prefer one of them, even if they are all equally correct. This paper shows that models such as CLIP have a \emph{task bias} where, given an image, their representations will prefer to solve one task over another one. 

%We identify this limitation of this zero-shot application paradigm\sm{remove this next bit?}.  We reveal that CLIP, the most widely used VLM, produces image representations strongly biased towards a particular task for a given image, often in unintuitive ways. 

This task bias is not an isolated phenomenon, and we show it occurs for most images. Such errors are a symptom of a deeper problem: it highlights that the visual representations of images with multiple potentially relevant tasks to be solved are specialized to one of these tasks, posing an issue for any downstream use of these representations. For instance, the popular DALL-E 2 text-to-image model \cite{ramesh_hierarchical_2022} is trained to invert the CLIP image encoder, but because the image encoder can selectively encode information about certain tasks and not others, this can lead DALL-E 2 to only consider information relevant to that task in its associated generations. We visualize this effect in Fig. \ref{fig:dalle2}. Attempting to engineer better text prompts to clarify the task cannot fix the problem because our results show that the bias exists in the visual representation before the categorical labels are considered.

We propose a straightforward solution to the task bias problem that requires no modification to the model parameters, making the fix widely applicable. We show that we can learn a visual prompt for each task that guide the image representations towards the task of interest, thereby addressing task bias. Figure \ref{fig:latents} illustrates the method. The prompt is independent of the image, and experiments show it steers the visual representation to focus on the task-relevant parts of the image. 

------


Time forpre-defined cate a quiz! eld graduate beyond Which of the choices in Fig.~\ref{fig:taskambimg} is correct for the image shown? With only the information provided, there is no clear answer; the action being performed is \textit{lift}, the text reads \textit{football}, and the most prominent object is a \textit{weight}. It is common sense that one cannot answer a question without a question. 
Yet the current paradigm has vision-language models (VLMs) such as CLIP \cite{radford_learning_2021} face decisions like this regularly in applied settings -- and, unknown to users, the models have already decided which question to answer solely from the image. As shown on the right of Fig.~\ref{fig:taskambimg}, when CLIP is given these choices, it has a strong bias to prefer one of them, even if they are all equally correct.

%If CLIP is given only valid choices, what do you think CLIP would pick given the quiz you just attempted?



The computer vision community often leverages large, hand-annotated datasets, such as the ImageNet benchmark \cite{russakovsky_imagenet_2015}. However, a new paradigm has emerged that capitalizes on corresponding image-text pairs on the Internet to learn deep visual representations without strong human supervision. Natural language supervision enabled the field to graduate beyond pre-defined categories, achieved excellent zero-shot performance, and even powered compositional generalization to out-of-distribution samples on various visual recognition tasks \cite{radford_learning_2021}.

Language has made computer vision accessible for many applications \cite{ramesh_hierarchical_2022,dhruv_paper,huypaper}. By naming a few categories in natural language (and not even labeling any images) the ascendant paradigm of ``zero-shot inference'' using these vision-language models enables the field to quickly build systems to recognize objects, actions, text, and anything else that can be described in language. It is this approach that has set the state-of-the-art on benchmarks. However, typically in these benchmarks, they will be given a classification problem where multiple answers are valid responses, the correct one only depending on the task. Consequently, there can be multiple answers that are equally correct, but associated with entirely different tasks. 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/latent_points_taskamb.pdf}
    \caption{(top) We show standard CLIP usage where an image is embedded into a multi-modal space, and the nearest word embedding is retrieved as the final answer. However, when there are multiple correct options, this approach has a \textit{task bias} where it prefers one task over the others. (bottom) We show to overcome this problem by learning a visual prompt that steers the representation towards the intended task.}
    \label{fig:latents}
\vspace{-1em}
\end{figure*}

This paper shows that models such as CLIP have a \emph{task bias} where, given an image, their representations will prefer to solve one task over another one.
%We identify this limitation of this zero-shot application paradigm\sm{remove this next bit?}.  We reveal that CLIP, the most widely used VLM, produces image representations strongly biased towards a particular task for a given image, often in unintuitive ways. 
This task bias is not an isolated phenomenon, and we show it occurs for most images. Following the standard zero-shot application procedure that language enables, models can thus solve tasks that were not intended by the user in realistic scenarios. Such errors are a symptom of a deeper problem: it highlights that the visual representations of images with multiple potentially relevant tasks to be solved are specialized to one of these tasks, posing an issue for any downstream use of these representations, such as in text-to-image models. For instance, the popular DALL-E 2 text-to-image model (also known as unCLIP) \cite{ramesh_hierarchical_2022} essentially is trained to invert the CLIP image encoder; because the image encoder can selectively encode information about certain tasks and not others, this can lead DALL-E 2/unCLIP to only consider information relevant to that task in its associated generations (see Fig. \ref{fig:dalle2}. Of course, attempting to engineer better text prompts to clarify the task cannot adjust the CLIP visual representations; we show that furthermore, it does not help even with guiding the predictions to a desired task.

% \vspace{-2.7em}
We propose a straightforward solution to the task bias problem that requires no modification to the model parameters, making the fix widely applicable. We show that we can learn a visual prompt for each task that guide the image representations towards the task of interest, thereby addressing task bias. Figure \ref{fig:latents} illustrates the method. The prompt is independent of the image, and experiments show it steers the visual representation to focus on the task-relevant parts of the image. 



\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/unclip.png}
    \caption{DALLE-2, or unCLIP, is trained using the CLIP visual representations, and can thus inherit the issue of task bias. This example, selected from \cite{ramesh_hierarchical_2022}, highlights that the generative model can primarily include information relevant to text in an image (iPod, leading to devices with the Apple logo) rather than information about the object present in the image that a user may want (a Granny Smith apple). }
    \vspace{-1em}
    \label{fig:dalle2}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

